MixDiff: Mixing Natural and Synthetic Images for Robust Self-Supervised Representations

This paper introduces MixDiff, a new self-supervised learning (SSL) pre-training framework that combines real and synthetic images. Unlike traditional SSL methods that predominantly use real images, MixDiff uses a variant of Stable Diffusion to replace an augmented instance of a real image, facilitating the learning of cross real-synthetic image representations. Our key insight is that while models trained solely on synthetic images underperform, combining real and synthetic data leads to more robust and adaptable representations. Experiments show MixDiff enhances SimCLR, BarlowTwins, and DINO across various robustness datasets and domain transfer tasks, boosting SimCLR's ImageNet-1K accuracy by 4.56%. Our framework also demonstrates comparable performance without needing any augmentations, a surprising finding in SSL where augmentations are typically crucial.

==> 02-background.tex <==
% \subsection{Self-supervised Learning}
% One of the most successful self-supervised learning paradigms is joint-embedding SSL. The main focus of joint-embedding SSL is instance-based discriminative learning~\cite{dosovitskiy2014discriminative, assran2023self}, where each image is considered to be its own class, and a model is trained by discriminating different views of the same image generated using data augmentation~\cite{moco,simclr,barlow,dino}. One such example is SimCLR~\cite{simclr}, which uses an InfoNCE-based formulation to bring in representation of different views of the same image closer (`positive pairs'), and repel representations of views from different images (`negative pairs') apart. In most cases, such joint-embedding SSL methods work in a Siamese setting where two branches have identical architectures and share weights. However, networks under such Siamese setting are
% vulnerable to collapsing to trivial representations. BarlowTwins~\cite{barlow} brings covariance regularization to the contrastive setting as a to enforce a non-collapsing solution. More recently, works such as DINO~\cite{dino} have shown alternative ways to precent collapse using architectural strategies inspired by knowledge distillation~.

% Given an unlabelled dataset $D = \{x_1, x_2...x_n\}$ where $x_i \in X \subset R^d$, represents the $i^th$ input. Any SSL method involves designing a pretext-task $S$ which utilizes pseudo-labels/feature representations $v_i \in Y$. We train a model $f(x)$ on $D_{train} \subset D$ such that $P(v|x)$, i.e. the conditional distribution of pseudo-labels given the input satisfies the pre-text task $S$. Eventually, we freeze the learned model parameters and train linear classifiers $g(f(x))$ on top of the model. The linear classifier is trained in a supervised manner via empirical risk minimization, $L(g(f(x)), y)$, where $y$ is the ground truth labels and $L$ is the training objective.

% \subsection{Diffusion Models for synthetic image generation}
